Providing Insights for Queries affected by Failures and Stragglers

Interactive time responses are a crucial requirement for users analyzing large amounts of data. Such analytical queries are typically run in a distributed setting, with data being sharded across thousands of nodes for high throughput. However, providing real-time analytics is still a very big challenge; with data distributed across thousands of nodes, the probability that some of the required nodes are unavailable or very slow during query execution is very high and unavailability may result in slow execution or even failures. The sheer magnitude of data and users increase resource contention and this exacerbates the phenomenon of stragglers and node failures during execution. In this paper, we propose a novel solution to alleviate the straggler/failure problem that exploits existing efficient partitioning properties of the data, particularly, co-hash partitioned data, and provides approximate answers along with confidence bounds to queries affected by failed/straggler nodes. We consider aggregate queries that involve joins, group bys, having clauses and a subclass of nested subqueries. Finally, we validate our approach through extensive experiments on the TPC-H dataset.

==> approximable.tex <==
\subsection{Approximable Queries}
\label{subsec:approximable}

==> cohash.tex <==
\section{How to Co-hash Partition?}
\label{sec:cohash}

In this section, we propose a co-hash partitioning design heuristic for a given workload, with the goal of maximizing the accuracy of approximate answers for the queries in a given workload. We first establish the accuracy difference of a partitioning design with respect to the `ideal' partitioning, which is obtaining a uniform random sample of the result of the query. There are two factors that contribute to this:

\begin{packed_item}
\item {\bf Cluster size variance}:  we quantify this using the formula $\frac{V_{Clustered}}{V_{SimpleRandomSample}} = \bar{N} \cdot (\frac{cv_N}{cv_y})^2 $ from~\cite{bookSarndal}. Here, $\bar{N}$ is the mean cluster size, $cv_{N}$ is the coefficient of cluster size variation, and $cv_{y}$ represents the coefficient of within cluster variance. 

\item {\bf Number of stages in the sample}: We represent the number of stages by $g$, and we estimate the contribution of correlation to the variance by $\Sigma_{k=1}^{K} \frac{(N-1)^{K-k}}{N^K}$, where $N$ is the number of clusters~\cite{crossJoin}.
\end{packed_item}

A database sample of a pre-determined size corresponding to a partitioning design can be used to estimate the above costs. We now define a simple partitioning accuracy metric:

\begin{definition} [Partitioning Cost]
The partitioning cost of a co-hash scheme $H$ for a given query $Q$, represented by $\mathcal{C}^H_Q$, is defined as $\sum_g \frac{V_{Clustered}}{V_{SimpleRandomSample}} + \Sigma_{k=1}^{K} \frac{(N-1)^{K-k}}{N^K}$.
For a workload $W: \{Q_1, \ldots, Q_m\}$, $\mathcal{A}^P_W$ is given by $\sum_{Q_i \in W} \mathcal{C}^H_{Q_i}$.
\end{definition}

Using techniques similar to~\cite{locationAware}, we now propose a novel algorithm to partition a given schema graph for a given workload $W$. From the above defined partitioning cost, we can see that the cost of having multiple stages far exceeds the cost of clustering the data. Hence, data locality is the primary factor to optimize for. Note that this is also the primary factor that determines the cost of running queries exactly~\cite{locationAware}. 

The first step in the algorithm is to annotate the schema graph with weights for edges. For each edge, the weight is defined as the cost of performing a network join, which is the size of the smaller table, multiplied by the number of times the join is used in the workload. In the second step, we obtain a MAST (Maximum Acyclic Spanning Tree) of the highest weight from the annotated schema graph. If there are multiple MASTs with the same weight, then we will perform the third step for each of the obtained MASTs. 

Finally, from the MAST, we enumerate all possible partitioning configurations by seeding each table in the MAST as the root table. The partitioning configurations should be \emph{relation non-redundant} and are allowed to be \emph{tuple redundant}. We obtain similar sized cluster samples of the database for each partitioning configuration $H$, determine $\mathcal{C}^H_W$, and finally choose the co-hash scheme $H$ that has the minimum cost. 

\tikzset{
    %Define style for boxes
    table/.style={
           rectangle,
           rounded corners,
           draw=black, thick,
           minimum height=2em,
           text centered},
    % Define arrow style
    pil/.style={
           shorten <=2pt,
           shorten >=2pt,}
}

\begin{figure}[!tbh]
\begin{subtable}{0.1\textwidth}
\scriptsize
\centering
\begin{tabular}{|c|c|}
\hline
Design & Hierarchies\\
\hline
$D_1$ & $H_6, H_7, H_{11}$\\
$D_2$ & $H_3, H_9, H_{11}$\\
$D_3$ & $H_{13}, H_7, H_{11}$\\
$D_4$ & $H_1, H_3, H_7, H_{11}$\\
$D_5$ & Replicate\\
$D_6$ & Figure~\ref{fig:design6}\\
\hline
\end{tabular}
\caption{\small{Partitioning Designs}} 
\label{tab:designs}
\end{subtable}%
\begin{subfigure}{0.5\textwidth}
\centering
\resizebox{0.55\linewidth}{!}{
\begin{tikzpicture}[node distance=1.5cm, auto]

 %nodes
 \node[table, fill=orange!20] (C) {\texttt{Customer}};
 \node[table, right=of C, fill=orange!20] (O) {\texttt{Order}};
 \node[table, right=of O, fill=orange!20] (L) {\texttt{Lineitem}};
 \node[table, below=of L,fill=orange!20] (P) {\texttt{Partsupp}};
 \node[table, below=of P,fill=orange!20] (PS) {\texttt{Part}};
 \node[table, below=of O,fill=orange!20] (S) {\texttt{Supplier}};
 \node[table, below=of C, dotted] (N) {\texttt{Nation}};
 \node[table, below=of N, dotted] (R) {\texttt{Region}};
 
 \path (C) edge[->,pil,thick] node {1.05 B} (O) ;
 \path (C) edge[pil,dotted] node {\scriptsize nationkey} (N) ;
 \path (N) edge[pil,dotted] node {\scriptsize regionkey} (R) ;
 \path (O) edge[->,pil,thick] node {15 M} (L) ;
 \path (N) edge[pil,dotted] node {\scriptsize nationkey} (S) ;
 \path (L) edge[<-,pil,thick] node {1 M} (P) ;   
 \path (PS) edge[->,pil,thick] node {800 K} (P) ; 
  \path (P) edge[pil,dotted] node {40 K} (S) ;
 \path (S) edge[->,pil,thick] node {50 K} (L) ; 
% \path (L) edge[pil,dotted,bend left=55] node[text width=0.6cm] {\scriptsize suppkey partkey} (P) ; 
\end{tikzpicture}}
\caption{\small{Design 6}} 
\label{fig:design6}
\end{subfigure}
\caption{\small{Partitioning designs with an example}}
\label{fig:partdesigns}
\end{figure}

\begin{example}
Consider the TPC-H benchmark that has 22 queries; the schema graph is depicted in Figure~\ref{fig:tpchJoinGraph}. Queries 2, 11, 15, 16, 20, and 22 have nested query predicates that access an entire relation (such as min and max) and this cannot be handled by the ASAP framework. Using the remaining queries, the edge weights are as shown in Figure~\ref{fig:design6}. 
%$Customer \Join Orders: 150 K \cdot 7$, $Lineitem \Join Orders: 1.5 M \cdot 10$, $Lineitem \Join Part: 200 K \cdot 5$, $Part \Join PartSupp: 200 K \cdot 4$, $Lineitem \Join Supplier: 10 K \cdot 5$, $Lineitem \Join Partsupp: 800 K \cdot 1$, $Supplier \Join PartSupp: 10 K \cdot 4$. 

Ignoring the edge directions in the tree in Figure~\ref{fig:design6} depicts the MAST that we will obtain from the schema graph. As part of the final step, we will use each table as the seed to enumerate different partitioning configurations. The partitioning configuration with the least cost has {\tt{Lineitem}} as the root relation; we call this Design 6 ($D_6$). A query Q that is approximable by $D_6$ has $\mathcal{C}^P_Q = 1$.
Observe that $D_6$ is relation non-redundant, but tuple redundant. Among relation non-redundant and tuple non-redundant partitioning schemes, $D_1 = \{H_6, H_7, H_{11}\}$ has the least cost; this is due to the frequent use of the $Order \Join Lineitem$ and $Customer \Join Order$ joins in the TPC-H queries.
\end{example}


%We now propose a heuristic for choosing a co-hash scheme for a database. From the previous discussion (Section~\ref{sec:estimators}), we observe that while co-locating helps queries that involve joins between the co-located tables, it may decreases accuracy for queries that involve tables that form a subgraph of the hierarchy. As as case in point, $H_6$ can improve the accuracy for query 3 in TPC-H, but can decrease the accuracy for query 6.

The second observation is, in the presence of skew, co-hashing
tables may adversely impact the accuracy for queries that do
not involve a join of the co-hashed tables. For example, for
the skewed data-set, design $D_2$ provided higher errors than
Indep. design for both queries 3 and 6. Additionally, we observe that 
the chosen co-hash scheme determines which queries with 
nested aggregates can be approximated.

%We propose a heuristic that decides on a co-hash partitioning strategy based on a given workload and database schema. The heuristic examines the hierarchies present in the queries of the workload; the more a hierarchy is used across queries, the more the benefit in having the hierarchy as part of the final partitioning design. The steps are as follows: For a given workload and schema, (a) enumerate all possible hierarchies in a given schema, (b) count the occurrences of hierarchies in the queries of the workload, and (c) greedily choose disjoint hierarchies that have the highest counts. We illustrate the application of this heuristic with an example below.
%%
%\begin{example}
%\label{ex:cohash}
%The TPC-H benchmark has 22
%queries; queries 2, 4, 11, 15, 16, 17, 18, 20, 21, and 22 have
%nested sub-queries. Queries 2, 11, 15, 16, 20, and 22 have nested query predicates that access an entire relation (such as min and max) and this cannot be handled by the ASAP framework.
%
%Using the remaining 16 queries from the TPC-H benchmark as the
%workload, we count the occurrences of hierarchies across 16
%queries. Barring single tables, $H_6$ occurs the most times.
%After we choose $H_6$, the remaining hierarchies that have more than
%one table are $H_7$ and $H_8$ with identical number of
%occurrences. Choosing $H_7$, followed by $H_{11}$, leads to design
%$D_1 = \{H_6, H_7, H_{11}\}$.
%%For queries with nesting, $D_1$ can approximate queries 4, 18 and 21. Had we chosen design $D_2 = \{H_3, H_8, H_{9} \}$, then query 17 can be approximated, but not 4, 18, and 21.
%\end{example}

==> efficiency.tex <==
\section{Accuracy vs Efficiency}
\label{sec:efficiency}

Aggregating Attribute and Homogeneity:
Given the estimators and their variances, the attributes that are used for aggregation determine the quality of the estimator and the magnitude of the variance obtained.
We will first define the term \emph{homogeneity} for a cluster in a given table. For a given aggregating attribute, if the intra-cluster variance is much lower than the inter-cluster variance, then the cluster is said to be homogeneous; homogeneous clusters contribute to high variance.
If the aggregating attribute is a partitioning attribute, then variance will be high, whereas aggregating over a non partitioning attribute will provide lower variance. If the aggregating attributes forms a subset of the partitioning attributes, then, the variance depends on the cluster sizes and the homogeneity of the clusters. An interesting point to note is that if there is no correlation between the partitioning attributes and the aggregating attributes, then the samples can be effectively viewed as tuple level sampling instead of cluster level sampling. However, it should be noted that the formulas given for computing variances take into account the worst case scenarios of the aggregating values being tightly correlated with that of the partitioning attribute. Under section~\ref{sec:eval}, we present experimental results to illustrate the ill effects of underestimating variance.

Also, as observed in the TPC-H and TPC-DS query templates, the aggregating attributes are generally real valued numbers that are not suitable for partitioning or joining, and the potential partitioning attributes are generally the join attributes.

==> labels.tex <==
\section{Labeling Results}
\label{sec:label}

One of the benefits of the $m$-table representation system is that it has information about the
dependency of tuples/values in the result on missing data. This information can be used 
to label the trustworthiness of tuples and attribute values in the result; in our previous
work we have discussed algorithms for obtaining labels for $m$-tables under $\pRA$.
In this section we extend the algorithms so as to obtain labels for $m$-tables that are extended 
to handle aggregates.

==> multisage.tex <==
\subsection{Optimizing for Accuracy}
\label{sec:singleOpt}

For efficiency, it is generally preferable to obtain the fewest
samples that provide the desired accuracy. This means that if there
are two samples that provide the same accuracy, and the size of one
sample is bigger than the other, the smaller size sample would be
preferred.  For such a case, it is possible to obtain the approximate
result with the desired accuracy more efficiently using multi-stage
sampling methods as opposed to single-stage
sampling~\cite{citeSomethingHer?}.  Bi-level sampling/multi-stage
sampling provides better variance than cluster sampling. The
higher variance in cluster sampling is due to variation in the sizes
of the clusters and due to homogeneity of the values in the clusters.

As we will discuss later, for tables that are co-hash partitioned into
a hierarchy, this is similar to the Wander Join algorithm for
approximating results~\cite{wanderJoin}. Another related sampling
scheme is the bi-level Bernoulli sampling scheme~\cite{bilevel} where,
given a table $T$, its pages are sampled with probability $p_i$ and
the rows are sampled with probability $q_i$, leading to an effective
sampling probability of $p = p_i q_i$ for $T$. There are multiple
differences between the bi-level (or multi-stage) sampling proposed
here and that proposed in~\cite{bilevel}; we discuss this in detail in
Section~\ref{sec:related}.

\subsection{Multi-stage Sampling}
In this section, we will first discuss two-stage sampling and
bi-level sampling and then generalize it to multi-stage
sampling. This will also provide the basis for discussing sampling
designs for approximating queries with joins.


\introparagraph{Bi-level Sampling:} For each table $T$ that needs to
be sampled we first determine two probabilities --- the first level
cluster sampling probability $(\pi_{Ii})$ and the second level cluster
(or tuple) sampling probability $(\pi_{k|i})$. Then $\pi_k =
\pi_{Ii} \cdot \pi_{k|i}$ is the effective sampling probability for
any element of $T_i$.

For tables that are hash partitioned on a unique attribute, $\pi_{Ii}$
equals 1 and $ \pi_{k|i}$ equals the ratio of number of tuples used
for processing to the total number of tuples. Since the table is
partitioned uniformly at random at the tuple level, there are no
\emph{clusters} in the sample.

For tables that are co-hash partitioned, we have $\pi_{Ii}$
equal to the ratio of the number of clusters sampled to the total number
of clusters. For sub-sampling at the second level, we can use a
predefined probability, $\pi_{k|i}$, for choosing elements (or
clusters) at the second level.  If we require cluster sampling for the
second level as well, we can choose any suitable attribute from the
table (or from any ancestor table along the join path for co-hashed
tables). Along with these probabilities, each table $T$ will now be
associated with the clustering attribute sets at the two levels; $B_T
= \{B_1, B_2\}$, where $B_1$ and $B_2$ are clustering attributes at
level 1 and level 2, respectively. In the case where the second level
does not involve cluster sampling, $B_2 = \emptyset$.


\introparagraph{Generalization to Multi-stage Sampling:} Extending the
bi-level sampling idea to multi-stage sampling with $k$ stages is
simple. For tables that are hash partitioned on an unique key, the
sampling probability for the first $k-1$ stages will be $1$.  For
other co-hash partitioned tables, the clustering attribute, $B_1$, and
the sampling probability, $\pi_{Ii}$, are predecided \em{Bruhathi:
  how???}. For the remaining $k-1$ stages, we need to pick suitable
clustering attributes, $B_i$, and decide on the sampling probability,
$p_i$, so that the resulting element sampling probability $\pi_k =
\pi_{Ii} \cdot \pi_{IIq|i} \ldots \cdot \pi_{k|iqr\ldots t}$.

This is especially applicable for co-hash partitioned hierarchies,
where tuples of tables are effectively clustered through join
attributes from other tables. For example, consider tables
{\tt{Customer, Orders}} and {\tt{Lineitem}} being co-hash partitioned
through the {\tt cust\_id} attribute of the {\tt Customer} table, as
illustrated in Table~\ref{tab:cohash}. Now, when choosing a
three-stage sample for {\tt Lineitem}, the clustering attribute of the
first stage is {\tt cust\_id}, the clustering attribute for the second
sampling stage can be chosen to be {\tt order\_id} and for the third
stage it can be {\tt line\_number} (equivalent to element level
sampling at the third level). This results in an efficient three stage
sampling technique for {\tt Lineitem} that does not involve random page
accesses.

\introparagraph{Multi-stage Sampling and Group Bys} Similar to the
case with cluster sampling, the effect of having Group-Bys on a
multistage sample depends on the attributes of the Group By and the
clustering attributes of the various stages of the multi-stage
sample. Let $G$ be the {\tt Group By} attributes and let $P = \bigcup
P_i$, where $P_i$ is the set of partitioning attributes at stage $i$
of the multi-stage sample, represent the set of partitioning
attributes across all stages.  Cases $G = P$ and $G \supset P$ follow
directly from the single table case. For case $G \cap P = \emptyset$,
we obtain multi-stage samples for each available group. For cases $G
\subset P$ and $G \not\subset P \land G \not\supset P$, once we obtain
$P-G$, we re-construct the partitioning attributes for the various
stages of the multi-stage sample. The cardinality of the partitioning
attribute set of some stages can be reduced. It is also possible that
$P_i = \emptyset$ for some stage $i$; in this scenario the number of
stages in the multi-stage sample will be reduced.






==> multistage.tex <==
\subsection{Optimizing for Accuracy}
\label{sec:singleOpt}

In scenarios where a desired accuracy or desired number of samples for a query is given by the user (continuously improving estimates are not required) and the cost of processing the obtained samples is high, it is preferable to obtain the fewest samples that provide the desired accuracy. 
%This means that between two samples that provide the same accuracy, if the size of one sample is bigger than the other, the smaller size sample is preferred, even if obtaining the bigger size sample is relatively cheaper.
For such a case, it is possible to obtain the approximate result with the desired accuracy more efficiently using multi-stage sampling methods.  Bi-level sampling/multi-stage sampling provide better variance than just cluster sampling. 
%As discussed in Section~\ref{subsec:accuracy}, the higher variance in cluster sampling is due to variation in the sizes of the clusters and due to homogeneity of the values in the clusters.
%As we will discuss later, for tables that are co-hash partitioned into a hierarchy, this is similar to the Wander Join algorithm for approximating results~\cite{wanderJoin}. 
% Page level sampling can be more efficient than row level sampling due to lower disk accesses; however, page level sampling may lead to large variances if intra-page values are homogeneous in comparison to inter-page values~\cite{samplingtutorial}. This trade-off was studied in detail in~\cite{bilevel}. 
%\subsection{Multi-stage Sampling}
In this section, we discuss multi-stage sampling. This will also provide the basis for discussing sampling designs for results obtained by joining multiple hierarchies. 


%\introparagraph{Bi-level sampling.}
%For each table or hierarchy, $H_i = (T_i, A_i)$, that needs to be sampled we first determine two probabilities -- the first level cluster sampling probability $(\pi_{Ii})$ and the second level cluster (or tuple) sampling probability $(\pi_{k|i})$. Further, $\pi_k = \pi_{Ii} \cdot \pi_{k|i}$ is the effective sampling probability for any element of $H_i$.
%
%For tables that are effectively hash partitioned on a unique attribute, $\pi_{Ii}$ equals 1 and $ \pi_{k|i}$ equals the tuple inclusion probability.
%%the ratio of number of tuples used for processing to the total number of tuples. Since the table is partitioned uniformly at random at the tuple level, there are no \emph{clusters} in the sample.
%% The number of tuples used for processing depends on the scenario; if it is a failure scenario resulting in incomplete data, then the number of tuples is the number of tuples of the table that are available; if it is the online aggregation scenario, then the number of tuples equals the number of tuples currently processed.
%For tables that are co-hash partitioned, we have $\pi_{Ii}$ equal to the cluster inclusion probability. For sub-sampling at the second level, we can use a predefined probability, $\pi_{k|i}$, for choosing tuples (or clusters) at the second level.  If we require cluster sampling for the second level as well, we can choose any suitable attribute set for clustering from the hierarchy $H_i$.
%%(or from any ancestor table along the join path for co-hashed tables). 
%Along with the inclusion probabilities, each table hierarchy $H_i$ will now be associated with clustering attribute sets at the two levels, $C_{H_i} = \{B_1, B_2\}$; note that $B_1 = A_i$.  
%%where $B_1$ and $B_2$ are clustering attributes at level 1 and level 2, respectively. In the case where the second level does not involve cluster sampling, $B_2 = \emptyset$.


\introparagraph{Multi-stage sampling.}
%Generalizing to multi-stage sampling with $k$ stages is simple. 
%For tables that are hash partitioned on an unique key, the sampling probability for the first $k-1$ stages will be $1$.  
Obtaining a multi-stage sample with $k$ stages is simple.
For co-hashed hierarchies, the clustering attribute, $B_1$, and the sampling probability, $\pi_{Ii}$, are predecided for the first stage. For the remaining $k-1$ stages, we need to pick suitable clustering attributes, $B_i$, and decide on the sampling probability, $p_i$, so that the resulting element sampling probability $\pi_k = \pi_{Ii} \cdot \pi_{IIq|i} \ldots \cdot \pi_{k|iqr\ldots t}$. This is especially applicable for co-hash partitioned hierarchies that involve multiple tables. Along with the inclusion probabilities, each hierarchy $H_i$ will now be associated with clustering attribute sets at the $k$ levels, $C_{H_i} = \{B_1, \ldots B_k\}$; note that $B_1 = A_i$.  

Consider the hierarchy $H_6$, whose partitioning is explicitly illustrated in Table~\ref{tab:cohash}. The clustering attribute of the first stage is {\tt c\_custkey}. We can choose a three-stage sample for {\tt Lineitem} by setting the clustering attributes of the second and third stages to be {\tt o\_orderkey} of table {\tt Orders} and {\tt l\_linenumber} of table {\tt Lineitem}, respectively. This results in an efficient three stage sampling technique for {\tt Lineitem} that doesn't involve random page accesses. 


\introparagraph{Multi-stage sampling and group bys.}
Similar to the case of cluster sampling, the effect of having Group-Bys on a multistage sample depends on the attributes of the Group By and the clustering attributes of the various stages of the multi-stage sample. Let $G$ be the {\tt Group By} attributes and let $ C_{H_i}$ represent the set of partitioning attributes across all stages. 
Cases $G = C_{H_i}$ and $G \supset C_{H_i}$ follow directly from the single table case. For case $G \cap C_{H_i} = \emptyset$, we obtain multi-stage samples for each available group. For cases $G \subset C_{H_i}$ and $G \not\subset C_{H_i} \land G \not\supset C_{H_i}$, once we obtain $C_{H_i}-G$, we re-construct the partitioning attributes for the various stages of the multi-stage sample. The cardinality of the partitioning attribute set of some stages can be reduced. It is also possible that $B_j \in C_{H_i} = \emptyset$ for some stage $j$; in this scenario the number of stages in the multi-stage sample will be reduced. 

%
%The variance formulas compute the worst case accuracy for a given data-set. For some queries in the TPC-H data-set, we can use the simpler formulas due to lack of correlations, and obtain higher accuracy. For some queries, we observed that computing the variance while treating the sample as an uniform random sample closely matched the variance observed experimentally. However, in some cases, it is hard to determine if this simplification can be done; for some highly selective queries, we observed that the variance computed with the formula closely matched the variance observed experimentally over 100 trials and treating the sample as uniformly random would have underestimated the variance.





==> singletable.tex <==
\subsection{Aggregates over Single Hierarchy}
\label{sec:singletable}

Obtaining approximate results for aggregates queries over single tables and over joins that only involve tables within a hierarchy follow the same procedure. We obtain a subset of data from the table (or from the intermediate result in case of a hierarchy) as described in Section~\ref{sec:framework}. For simple aggregates, the data obtained will be a cluster sample and we use the methods described in Section~\ref{sec:sampling} to obtain estimations and confidence bounds for the aggregates. We now describe obtaining confidence bounds in the presence of the {\tt GROUP BY} operator.

\introparagraph{Group By.}
The effect of co-hash partitioning on the results of the {\tt GROUP BY} operation depends on the relationship between the co-hash partitioning attributes and the {\tt GROUP BY} attributes. If $G$ represents the {\tt GROUP BY} attributes and the query involves tables from a hierarchy $(T, A)$, where $A$ represents the clustering/partitioning attributes of the hierarchy, then we have 3 possible cases:
\begin{packed_enum}
\item {\bf{$G=A$}}: In this case, the result could be missing some groups, but the groups that are present in the result will be the exact aggregate value.

\item {\bf{$G \cap A = \emptyset$}}: This is similar to approximating simple aggregates. For each group that is present we will obtain cluster samples that are clustered by $A$.

\item {\bf{$ G \cap A \neq \emptyset$}}: There are three subcases:
\begin{packed_enum}
\item {\bf{$G \supset A $}}: This subcase is similar to case 1; there will be some groups missing, but for the groups that are present, the result will be the true aggregate value.
\item {\bf{$G \subset A $}}: This subcase is similar to approximating simple aggregates. For each group that is present we will obtain cluster samples that are clustered by $A-G$.
\item  {\bf{$G \not\subset A \land G \not\supset A$}}: This is the tricky case, where we have some common attributes between the partitioning attribute set and the group by attribute set; but, the result is similar to the previous case, where in each group that is present will have cluster samples that are clustered by $A-G$.
\end{packed_enum}

\end{packed_enum}

\begin{example}
Consider a TPC-H data set co-hash partitioned as given in Figure~\ref{fig:hierarchy}, consisting of hierarchies $H_6, H7$ and $H_{11}$. Now, query 3 of the benchmark involves a join between all three tables of hierarchy $H_6$, and a group by operation on attributes {\tt l\_orderkey, o\_orderdate,} and  {\tt o\_shippriority}. Since $H_6$ is clustered on {\tt c\_custkey}, this falls under case 2, where $G \cap A \neq \emptyset$.
\end{example}

\introparagraph{Nested Aggregates.}
When nested aggregates are over ``complete" values (only missing groups, but the aggregate values for the groups that are present are accurate), then computing nested aggregates is the same as computing simple aggregates over subset of data. 
This can occur under two situations: $(i)$ the predicates are on the aggregate values obtained by the {\tt GROUP BY} operation and the operation falls under cases 1 or 3(b) above, and $(ii)$ the nested aggregate/predicate references tuples that are co-located, and hence, each value obtained is ``complete". 
However, when the group aggregates are themselves approximate values, it is not immediately clear how to obtain an approximate value over approximate values. 

\begin{example}
Consider a TPC-H dataset that is co-hash partitioned resulting in ${({\tt Customer} \leftarrow {\tt Orders}  \leftarrow {\tt Lineitem}, {\tt c\_custkey})}$ as one of the co-hashed hierarchies. Now, consider query 4 from the benchmark, that counts the number of orders that have at least one lineitem with a given {\tt commitdate}. This cannot be approximated easily, but with the above co-hashed hierarchy, all lineitems of a order are co-located, and hence, we can obtain an approximate count of orders that satisfy the given predicate.
\end{example}


